Deep Paper Gestalt

Recent years have witnessed a significant increase in the number of paper submissions to computer vision conferences. The sheer volume of paper submissions and the insufficient number of competent reviewers cause a considerable burden for the current peer review system. In this paper, we learn a classifier to predict whether a paper should be accepted or rejected based solely on the visual appearance of the paper (i.e., the gestalt of a paper). Experimental results show that our classifier can safely reject 50% of the bad papers while wrongly reject only 0.4% of the good papers, and thus dramatically reduce the workload of the reviewers. We also provide tools for providing suggestions to authors so that they can improve the gestalt of their papers.

==> conclusion.tex <==
\section{Conclusions}
\label{sec:conclusions}

% Briefly summarize what we did in this work.

% Disclose all limitations

% Describe how potential future work can address these limitations and lead to interesting and ground breaking stuff.

==> figure/fig_overview.tex <==
\begin{figure*}[t]
\jbox{\textwidth}{0.3\textwidth}
\caption{Overview of the method.}
\label{fig:overview}
\end{figure*}

==> figure/fig_teaser.tex <==
\begin{center}
    \centering
    \jbox{\textwidth}{0.3\textwidth}
    \captionof{figure}{Teaser figure. Main idea of the paper.}
    \label{fig:teaser}
\end{center}

==> overview.tex <==
\section{Overview}
\label{sec:overview}

% Introduce your problem with a toy example

% This figure illustrate the overall process of the algorithm, starting from inputs, processing steps, and outputs. Use forward references the figures with the corresponding equations and sections in the paper.
\input{figure/fig_overview}

==> result.tex <==
\section{Experimental Results}
\label{sec:results}

\subsection{Datasets}
% Describe datasets used, statistics (# images, train/test splits)

\subsection{Evaluation metrics}
% Describe how you evaluate the performance

\subsection{Implementation details} 
% Reveal ALL parameter values, running time (including machine specs), and any other tricks described in the paper.

\subsection{Quantitative evaluation}
% Comparison to the state-of-the-art

\subsection{Qualitative evaluation}
% Show visual results

\subsection{Ablation study}
% Evaluate the individual contribution of each component

\subsection{Failure modes}
% Show failure cases and discuss potential ways for improving it.

